Team voyTECH: User Activity Modeling with Boosting Trees

This paper describes our winning solution for the ECML-PKDD ChAT Discovery Challenge 2020. We show that whether or not a Twitch user has subscribed to a channel can be well predicted by modeling user activity with boosting trees. We introduce the connection between target-encodings and boosting trees in the context of high cardinality categoricals and find that modeling user activity is more powerful then direct modeling of content when encoded properly and combined with a suitable optimization approach.

==> symbols.tex <==


\long\def\ignore#1{}

%Results
%Shortcuts
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
%\newcommand{\A}{\mathbf{A}}
\newcommand{\bi}{\mathbf{b}}
\newcommand{\ro}{\mathbf{r}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\ep}{\epsilon}
\newcommand{\de}{\delta}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   General notation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Epsilon
\newcommand{\eps}{\varepsilon}

% Extended condition number of A (J. Demmel)
\newcommand{\kappaFS}{\kappa^2_{\textrm{\tiny F}}}
\newcommand{\kappaF}{\kappa_{\textrm{\tiny F}}}



% Absolute Value of a number
\newcommand{\abs}[1]{\left|#1\right|}

% Optimum
\def\opt{{\textrm{opt}}}

% Polynomial factors
\newcommand{\poly}[1]{\mathrm{poly}\left(#1\right) }

% Polylog(n)
\newcommand{\polylog}[1]{\ensuremath{\operatorname{polylog}\left(#1\right)}}

\newcommand{\sign}[1]{\ensuremath{\operatorname{\textbf{sign}}\left(#1\right)}}
% Big-Oh Notation
\newcommand{\OO}{\mathcal{O}}

% Volume of a set
\newcommand{\vol}[1]{\operatorname{vol}(#1)}

% Set of categoricals
\newcommand{\CC}{\mathcal{C}}
% Caligraphic subset
\newcommand{\CS}{\mathcal{S}}


% Real numbers
\newcommand{\RR}{\mathbb{R}}
\newcommand{\reals}{\mathbb{R}}

% Integers numbers
\newcommand{\ZZ}{\mathbb{Z}}

% Natural numbers
\newcommand{\NN}{\mathbb{N}}

% Euler's constant
\newcommand{\e}{\ensuremath{{\textrm e}}}

% Sparsity of matrix
\newcommand{\ravg}{\mathrm{R}_{\mathrm{avg}}}
\newcommand{\cavg}{\mathrm{C}_{\mathrm{avg}}}

% Expectation
\DeclareMathOperator{\EE}{\mathbb{E}}

% Probability
\newcommand{\Prob}[1]{\ensuremath{\mathbb{P}\left(#1\right)}}
% Variance
\newcommand{\var}[1]{\ensuremath{\mathrm{Var}(#1)}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Several norms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\norm}[1]{\ensuremath{\left\|#1\right\|_2}}
\newcommand{\pnorm}[1]{\ensuremath{\left\|#1\right\|_p}}
\newcommand{\qnorm}[1]{\ensuremath{\left\|#1\right\|_q}}
\newcommand{\infnorm}[1]{\ensuremath{\left\|#1\right\|_\infty}}
\newcommand{\onenorm}[1]{\ensuremath{\left\|#1\right\|_1}}
\newcommand{\frobnorm}[1]{\ensuremath{\left\|#1\right\|_{\textrm{F}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%=======================
%% Matrix quantities
%=======================
%=======================
% Stable rank of a matrix
\newcommand{\sr}[1]{\ensuremath{\operatorname{\textbf{\footnotesize sr}}\left(#1\right)}}
% Trace of a matrix.
\newcommand{\trace}[1]{\ensuremath{\operatorname{\textbf{tr}}\left(#1\right)}}
%\DeclareMathOperator{\trace}{trace}
% Rank of a matrix
\newcommand{\rank}[1]{\ensuremath{\operatorname{\textbf{{\footnotesize rank}}}\left(#1\right)}}
% Kernel of a matrix
%\newcommand{\ker}[1]{\ensuremath{\mathrm{\textbf{ker}}\left(#1\right)}}
% Image of a matrix
\newcommand{\im}[1]{\ensuremath{\operatorname{\textbf{Im}}\left(#1\right)}}
% Condition number of a matrix
\newcommand{\cond}[1]{\ensuremath{\operatorname{\mathrm{cond}}\left(#1\right)}}
% Matrix exponential
\newcommand{\expm}[1]{\ensuremath{\operatorname{\textbf{\footnotesize exp}}\left[#1\right]}}
% Matrix Hyperbolic Cosine
\newcommand{\coshm}[1]{\ensuremath{\operatorname{\textbf{\footnotesize cosh}}\left[#1\right]}}
% Determinant
\newcommand{\detm}[1]{\ensuremath{\operatorname{\textbf{det}}\left(#1\right)}}
% Pseudo-inverse of a matrix
\newcommand{\pinv}[1]{ {#1}^\dagger}

% Pseudo-inverse of a matrix
\newcommand{\tpinv}[1]{ {#1}^{\dagger\top}}
% # of non-zero entries of a matrix
\newcommand{\nnz}[1]{\ensuremath{\operatorname{\textbf{\footnotesize nnz}}\left(#1\right)}}
% Diagonal Matrix
\newcommand{\diag}[1]{\ensuremath{\operatorname{\textbf{diag}}\left(#1\right)}}
% Column span of a matrix
\newcommand{\colspan}[1]{\mathcal{R}(#1)}
% The dilation of a matrix
\newcommand{\dil}[1]{\ensuremath{\mathcal{D}\left(#1\right)}}
%=======================
%=======================


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Vector and matrix operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% Inner product
\newcommand{\ip}[2]{\left\langle {#1},\ {#2} \right\rangle}
% Matrix inner product ( A \bullet B := tr(AB)
\newcommand{\mip}[2]{ {#1}\bullet {#2}}



% Special matrices (CONSTANTS)
\newcommand{\Id}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\onemtx}{\bm{1}}
\newcommand{\zeromtx}{\mathbf{0}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mat}[1]{ {\ensuremath{\mathsf{#1} }}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\gammab{{\bm{\gamma}}}
\def\kappab{{\bm{\kappa}}}
\def\sig{{\bm{\Sigma}}}
\def\sigplus{{\bm{\Sigma}^{+}}}
\def\siginv{{\bm{\Sigma}^{-1}}}
\def\bet{{\bm{\beta}}}
\def\one{{\bm{1}}}
\def\exp{\hbox{\textrm exp}}
\def\col{\hbox{\textrm col}}
\def\ker{\hbox{\textrm ker}}
\def\ahat{{\hat\a}}
\def\p{{\mathbf p}}
\def\e{{\mathbf e}}
\def\q{{\mathbf q}}
\def\rb{{\mathbf r}}
\def\s{{\mathbf s}}
\def\u{{\mathbf u}}
\def\v{{\mathbf v}}
\def\d{{\mathbf \delta}}
\def\xhat{{\hat\x}}
\def\yhat{{\hat\y}}
\def\A{\matA}
\def\B{\matB}
\def\C{\matC}
\def\Ahat{\hat\matA}
\def\Atilde{\tilde\matA}
\def\Btilde{\tilde\matB}
\def\Stilde{\tilde\matS}
\def\Utilde{\tilde\matU}
\def\Vtilde{\tilde\matV}
\def\G{{\cl G}}
\def\hset{{\cl H}}
\def\Q{{\bm{Q}}}
\def\U{{\bm{U}}}
\def\V{{\bm{V}}}
\def\win{\hat{\w}}
\def\wopt{\w^*}
\def\matAhat{\hat\mat{A}}
\def\matA{\mat{A}}
\def\matB{\mat{B}}
\def\matC{\mat{C}}
\def\matD{\mat{D}}
\def\matE{\mat{E}}
\def\matG{\mat{G}}
\def\matH{\mat{H}}
\newcommand{\matI}{\Id} % This matrix is reserved for the Identity matrix
\def\matM{\mat{M}}
\def\matP{\mat{P}}
\def\matQ{\mat{Q}}
\def\matR{\mat{R}}
\def\matL{\mat{L}}

\def\matS{\mat{S}}
\def\matT{\mat{T}}
\def\matU{\mat{U}}
\def\matV{\mat{V}}
\def\matW{\mat{W}}
\def\matX{\mat{X}}
\def\matY{\mat{Y}}
\def\matZ{\mat{Z}}
\def\matSig{\mat{\Sigma}}
\def\matOmega{\mat{\Omega}}
\def\matGam{\mat{\Gamma}}
\def\matTh{\mat{\Theta}}

\newcommand{\matPi}{\mat{\Pi}}
\newcommand{\matPsi}{\mat{\Psi}}
\newcommand{\matPhi}{\mat{\Phi}}
\def\w{{\mathbf{w}}}
\def\ein{{\cl E_{\mathrm{in}}}}
\def\eout{{\cl E}}



\def\vecx{\vct{x}}
\def\vecb{\vct{b}}
\def\vecu{\vct{u}}
\def\vecy{\vct{y}}
\def\vecz{\vct{z}}
\def\veco{\vct{o}}
\def\vecw{\vct{w}}
\def\vecv{\vct{v}}
\def\vecp{\vct{p}}



%% CAUTION OVERRIDE NOTATION
% Over-ride notation
\def\b{{\mathbf b}}


\newcommand{\bc}{{\b_{\mathcal{R}(\matA)^\bot } }}
\newcommand{\br}{{\b_{\mathcal{R}(\matA) } }}

% Least squares solution of Ax = b
\newcommand{\xls}{\x_{\textrm{\tiny LS}}}
\newcommand{\xopt}{\x_{\textrm{\tiny opt}}}

\newcommand{\yls}{\y_{\textrm{\tiny LS}}}
\newcommand{\yopt}{\y_{\textrm{\tiny opt}}}

% For rows, columns and entries of a matrix A
\newcommand{\ar}[1]{ \matA^{(#1)}}
\newcommand{\ac}[1]{ \matA_{(#1)}}
\newcommand{\Ae}[1]{ \mat{a}_{#1}}

% For rows, columns and entries of a matrix B
\newcommand{\Br}[1]{ \matB^{(#1)}}
\newcommand{\Bc}[1]{ \matB_{(#1)}}
\newcommand{\Be}[1]{ \matB_{#1}}


% For rows and columns and entries of a matrix L
\newcommand{\Lr}[1]{ \matL^{(#1)}}
\newcommand{\Lc}[1]{ \matL_{(#1)}}
\newcommand{\Le}[1]{ \matL_{#1}}

% Normalized Laplacian
\newcommand{\Ln}{\matL_{\textrm{\tiny norm}}}
\newcommand{\Lnr}[1]{ \matL_{\textrm{\tiny norm}}^{(#1)}}
\newcommand{\Lnc}[1]{ \matL_{\textrm{\tiny norm}_{(#1)}}}
\newcommand{\Lne}[1]{ \matL_{\textrm{\tiny norm}_{#1}} }



% For rows, columns and entries of a matrix Q
\newcommand{\qr}[1]{ \matQ^{(#1)}}
\newcommand{\qc}[1]{ \matQ_{(#1)}}

% For rows, columns and entries of a matrix tilde Q
\newcommand{\tqr}[1]{ \widetilde{\matQ}^{(#1)}}
\newcommand{\tqc}[1]{ \widetilde{\matQ}_{(#1)}}





\newcommand{\argmin}{\operatorname*{arg\; min}}
\newcommand{\argmax}{\operatorname*{arg\; max}}

% Cayley Graph of a group G and subset S.
\newcommand{\Cay}[2]{\ensuremath{\operatorname{Cay}\left(#1; #2\right)}}


\newcommand{\Sym}{\mathcal{S}}


\newcommand{\myMat}[4]{\left[\begin{array}[c]{ll}
#1 & #2 \\
#3 & #4
\end{array}
\right]}


%Results
%Shortcuts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   General notation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Optimum
\def\opt{{\textrm{opt}}}


\def\gammab{{\bm{\gamma}}}
\def\kappab{{\bm{\kappa}}}
\def\sig{{\bm{\Sigma}}}
\def\sigplus{{\bm{\Sigma}^{+}}}
\def\siginv{{\bm{\Sigma}^{-1}}}
\def\bet{{\bm{\beta}}}
\def\one{{\bm{1}}}
\def\exp{\hbox{\textrm exp}}
\def\col{\hbox{\textrm col}}
\def\ker{\hbox{\textrm ker}}
\def\ahat{{\hat\a}}
\def\p{{\mathbf p}}
\def\e{{\mathbf e}}
\def\q{{\mathbf q}}
\def\rb{{\mathbf r}}
\def\s{{\mathbf s}}
\def\u{{\mathbf u}}
\def\v{{\mathbf v}}
\def\d{{\mathbf \delta}}
\def\xhat{{\hat\x}}
\def\yhat{{\hat\y}}
\def\A{\matA}
\def\B{\matB}
\def\C{\matC}
\def\Ahat{\hat\matA}
\def\Atilde{\tilde\matA}
\def\Btilde{\tilde\matB}
\def\Stilde{\tilde\matS}
\def\Utilde{\tilde\matU}
\def\Vtilde{\tilde\matV}
\def\G{{\cl G}}
\def\hset{{\cl H}}
\def\Q{{\bm{Q}}}
\def\U{{\bm{U}}}
\def\V{{\bm{V}}}
\def\win{\hat{\w}}
\def\wopt{\w^*}
\def\matAhat{\hat\mat{A}}
\def\matA{\mat{A}}
\def\matB{\mat{B}}
\def\matC{\mat{C}}
\def\matD{\mat{D}}
\def\matE{\mat{E}}
\def\matG{\mat{G}}
\def\matH{\mat{H}}
\def\matM{\mat{M}}
\def\matP{\mat{P}}
\def\matQ{\mat{Q}}
\def\matR{\mat{R}}
\def\matL{\mat{L}}

\def\matS{\mat{S}}
\def\matT{\mat{T}}
\def\matU{\mat{U}}
\def\matV{\mat{V}}
\def\matW{\mat{W}}
\def\matX{\mat{X}}
\def\matY{\mat{Y}}
\def\matZ{\mat{Z}}
\def\matSig{\mat{\Sigma}}
\def\matOmega{\mat{\Omega}}
\def\matGam{\mat{\Gamma}}
\def\matTh{\mat{\Theta}}

\def\w{{\mathbf{w}}}
\def\ein{{\cl E_{\mathrm{in}}}}
\def\eout{{\cl E}}



\def\vecx{\vct{x}}
\def\vecb{\vct{b}}
\def\vecu{\vct{u}}
\def\vecy{\vct{y}}
\def\vecz{\vct{z}}
\def\veco{\vct{o}}
\def\vecw{\vct{w}}
\def\vecv{\vct{v}}
\def\vecp{\vct{p}}

